AutoLay: Benchmarking amodal layout estimation for autonomous driving

Given an image or a video captured from a monocular camera, amodal layout estimation is the task of predicting semantics and occupancy in bird's eye view. The term amodal implies we also reason about entities in the scene that are occluded or truncated in image space. While several recent efforts have tackled this problem, there is a lack of standardization in task specification, datasets, and evaluation protocols. We address these gaps with AutoLay, a dataset and benchmark for amodal layout estimation from monocular images. AutoLay encompasses driving imagery from two popular datasets: KITTI and Argoverse. In addition to fine-grained attributes such as lanes, sidewalks, and vehicles, we also provide semantically annotated 3D point clouds. We implement several baselines and bleeding edge approaches, and release our data and code.

==> 01intro.tex <==
\section{Introduction}
\label{sec:introduction}



% The rest of this paper is organized as follows: Section \ref{relatedwork} discusses relevant work on predicting future states of the world. The proposed approach is detailed in Section \ref{sec:intermediate_representations} and  \ref{sec:approach}, Section \ref{sec:intermediate_representations} focusses on the intermediate representations: why they are important, what they capture what other representations do not, whereas Section \ref{sec:approach} focusses on the problem formulation, the network architecture and the training objective. An account of the dataset, experiments and results is provided in Section \ref{sec:results}, and the work is concluded in Section \ref{sec:conclusions}. \Krishna{This paragraph is usually boring, and people don't read it. IMO, could remove this entirely.}

==> 02relatedwork.tex <==
\section{Related Work} \label{relatedwork}



==> 03dataprep.tex <==
\section{The KITTI-Layout Dataset}
\label{sec:Dataset}


\section{Data Preparation: Weak Supervision}

==> 04approach.tex <==
\section{Layout Prediction with Temporal Consisitency}
\label{sec:approach}


==> 05results.tex <==
\section{Results}
\label{sec:results}


==> 06conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}




==> 07acknowledgements.tex <==
\section*{Acknowledgements}



==> 08DiscussionandFuture.tex <==
\section*{Discussion}


==> autolay-iros-2020 (1)/01intro.tex <==
\section{Introduction}
\label{sec:introduction}



% The rest of this paper is organized as follows: Section \ref{relatedwork} discusses relevant work on predicting future states of the world. The proposed approach is detailed in Section \ref{sec:intermediate_representations} and  \ref{sec:approach}, Section \ref{sec:intermediate_representations} focusses on the intermediate representations: why they are important, what they capture what other representations do not, whereas Section \ref{sec:approach} focusses on the problem formulation, the network architecture and the training objective. An account of the dataset, experiments and results is provided in Section \ref{sec:results}, and the work is concluded in Section \ref{sec:conclusions}. \Krishna{This paragraph is usually boring, and people don't read it. IMO, could remove this entirely.}

==> autolay-iros-2020 (1)/02relatedwork.tex <==
\section{Related Work} \label{relatedwork}



==> autolay-iros-2020 (1)/03dataprep.tex <==
\section{The KITTI-Layout Dataset}
\label{sec:Dataset}


\section{Data Preparation: Weak Supervision}

==> autolay-iros-2020 (1)/04approach.tex <==
\section{Layout Prediction with Temporal Consisitency}
\label{sec:approach}


==> autolay-iros-2020 (1)/05results.tex <==
\section{Results}
\label{sec:results}


==> autolay-iros-2020 (1)/06conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}




==> autolay-iros-2020 (1)/07acknowledgements.tex <==
\section*{Acknowledgements}



==> autolay-iros-2020 (1)/08DiscussionandFuture.tex <==
\section*{Discussion}


==> autolay-iros-2020 (1)/include/includepackages.tex <==
\usepackage{times}
\usepackage{blindtext, rotating}

\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}

\usepackage{tabularx}

\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{textcomp}
\usepackage{gensymb}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{float}
\usepackage{capt-of}
\usepackage{etoolbox}
\usepackage{adjustbox}
\usepackage[font=small]{caption}

\usepackage{paralist}

\usepackage[colorlinks=true, pagebackref]{hyperref}
% % Not including hyperref, as it does not play well with vision conference (CVPR/ICCV/WACV/3DV) styles.
% % If you comment hyperref and then uncomment it, you should delete
% % egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% % run, let it finish, and you should be clear).
% \usepackage[pagebackref=true,breaklinks=true,letterpaper=true,colorlinks,bookmarks=false]{hyperref}

% For the fancy quote in the beginning of the paper
\usepackage{epigraph}


==> autolay-iros-2020 (1)/include/mymacros.tex <==
% Macros for reviewing paper, marking todos
\newcommand{\TODO}[1]{{\color{red} \textbf{TODO: #1}}}
\newcommand{\Krishna}[1]{{\color{red}{\textbf{Krishna}: #1}}}
\newcommand{\Kaustubh}[1]{{\color{blue}{\textbf{Kaustubh}: #1}}}
\newcommand{\SaiShankar}[1]{{\color{green}{\textbf{SaiShankar}: #1}}}
\newcommand{\Madhav}[1]{{\color{magenta}{\textbf{MK}: #1}}}
\newcommand{\todo}[1]{{\color{red} \textbf{TODO: #1}}}

% Common abbreviations
\newcommand{\etal}{\emph{et al.}}
\newcommand{\cf}{\emph{cf.}}

% Text colors
\newcommand{\red}[1]{{\textcolor{red}{#1}}}
\newcommand{\blue}[1]{{\textcolor{blue}{#1}}}
\newcommand{\green}[1]{{\textcolor{green}{#1}}}
\newcommand{\gray}[1]{{\textcolor{gray}{#1}}}
\newcommand{\pink}[1]{{\textcolor{pink}{#1}}}


\newcommand{\monolayout}{\emph{MonoLayout}}
\newcommand{\videolayout}{\emph{VideoLayout}}
\newcommand{\bev}{bird's eye view}
\newcommand{\coolname}{\emph{AutoLay}}
\newcommand{\autolay}{\emph{AutoLay}}

% \newcommand{\mb}[1]{\mathbf{#1}}


% Math shorthand

% Shorthand for \mathbf
\newcommand{\mb}[1]{\mathbf{#1}}
\newcommand{\mcal}[1]{\mathcal{#1}}


==> autolay-iros-2020 (1)/text/approach.tex <==
 \section{Approach}
\label{sec:approach}



\begin{figure*}[!ht]
  \centering
  \includegraphics[width=\textwidth]{figures/weak_supervision_km.png}
  \caption{\textbf{Weak Supervision setup}: We show our automated (noisy) label generation scheme herein. Points from the lidar frame are projected down to semantically segmented images (a), to obtain sparse static layouts (b). These sparse layouts are stacked across an image sequence to generate dense static layouts (c). In the next step (d), road and lane boundaries are extracted and combined to obtain lane layouts (e).}
  \label{fig: weak_supervision}
\end{figure*}




% \Kaustubh{Write the overarching narrative for the entire approach section.(ConvLSTM, Consistency Loss, Refinement GAN)}



% \subsection{Network Architecture}

% % \subsubsection{Feature Extraction} 


% We use ResNet-18\Kaustubh{cite resnet} encoder(pretrained on ImageNet) in order to extract rich features at multiple-scales from a sequence of input images. 

Learning the mapping function described in Sec.~\ref{sec:problem} which maps the perspective RGB images to the static and dynamic layouts in \bev{} is quite a challenging problem. The problem demands an accurate understanding and modeling of the 3D scene which necessitates the requirement for learning good visual features that can encode the depth and the semantics of the 3D scene. Most approaches~\cite{schulter2018learning, monolayout, monooccupancy} to monocular layout estimation operate on a single RGB image input, which often leads to temporally inconsistent predictions.


In this section, we tackle the aforementioned problem by proposing a neural network architecture that takes a sequence of images as input and generates temporally consistent layouts as output. 

% the proposed \videolayout architecture 

% Amodal scene layout estimation is a challenging t


\subsection{\videolayout{}: Temporally Consistent Layout Estimation}
\label{subsec:videolayout}


% We formulate the problem of amodal scene layout prediction as estimating Maximum a posteriori corresponding to the distribution of static and dynamic scene participants. 

Given a sequence of RGB images $\mathcal{I}_1, \mathcal{I}_2, ..., \mathcal{I}_t$ as input, our model predicts the posterior distribution $P(\mathcal{S}_t, \mathcal{D}_t | {\mathcal{I}_1, \mathcal{I}_2, ..., \mathcal{I}_t})$, where $\mathcal{S}_t$ and $\mathcal{D}_t$ denote the predicted static and dynamic layouts corresponding to image $\mathcal{I}_t$. 


Our network architecture consists of four subparts:
\begin{itemize}
    \item A feature encoder which takes as input a sequence of RGB images $\mathcal{I}_1, \mathcal{I}_2, ..., \mathcal{I}_t$ and generates rich multi-scale features maps $\mathcal{C}_1, \mathcal{C}_2, ..., \mathcal{C}_t$ corresponding to each rgb image.
    
    \item A stacked Convolutional LSTM submodule which aggregates image features $\mathcal{C}_1, \mathcal{C}_2, ..., \mathcal{C}_t$  and encodes a temporal representation useful for estimating consistent layouts. 
    
    \item Similar to \cite{monolayout}, we maintain two set of decoder weights corresponding to the static and dynamic decoders. Both decoders share a similar architecture except for the use of sampling layer at the beginning of the static decoder in order to generate smooth looking road and lane layouts. Instead of directly processing the encoded output representation of convLSTM, we instead sample from a gaussian distribution with the feature map as the mean values and a fixed standard deviation. 
    
    % \SaiShankar{explain sampling layer}
    
    \item A Refinement Network, which helps in improving the quality of the output static and dynamic layouts by regularizing the predicted layouts in order to resemble the true data distribution.
\end{itemize}


% \Kaustubh{Write why temporal consistency is important and the failures of MonoLayout in maintaining temporal stability in its prediction.}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.9\linewidth]{figures/architecture.png}
%     \caption{\videolayout{} Architecture}
%     \label{fig:architecture}
% \end{figure}



\subsection{Consistency Loss}

The weights of the \videolayout{} architecture are updated via backpropagation using the loss function defined in Eq.~\ref{eq:total_loss}. 

\vspace{-1em}
\begin{equation}
    \mathcal{L}_{sup} = \sum_{i=1}^N f(\Bar{S}_i,  S_i) +  f(\Bar{D}_i,  D_i) 
\end{equation}

\vspace{-1.5em}
\begin{equation}
    \mathcal{L}_{short}^{c} = \sum_{i=1}^N \sum_{j=1}^{seqlen-1} f(\Bar{S}_i^j, \Bar{S}_i^{j+1}) + f(\Bar{D}_i^j, \Bar{D}_i^{j+1})
\end{equation}

\vspace{-1.5em}
\begin{equation}
    \mathcal{L}_{long}^{c} = \sum_{i=1}^N \sum_{j=1}^{seqlen-1} \sum_{k=j+2}^{seqlen} f(\Bar{S}_i^j, \Bar{S}_i^{k}) + f(\Bar{D}_i^j, \Bar{D}_i^{k})
\end{equation}

\vspace{-1.5em}
\begin{equation}
    \mathcal{L} = \lambda_{sup} * \mathcal{L}_{sup} + \lambda_{short}^c * \mathcal{L}_{short}^{c} + \lambda_{long}^c * \mathcal{L}_{long}^{c}
    \label{eq:total_loss}
\end{equation}
    
    
Here, $\Bar{S}$ and $\Bar{D}$ denote the predicted static and dynamic layouts respectively, $S$ and $D$ denote the ground truth (weak/strong) layouts. $N$ is the mini batch size, $seqlen$ is the length of the input image sequence per sample. $f(\cdot, \cdot)$ is the cross-entropy loss function. $\mathcal{L}_{sup}$ is a supervised loss term that penalizes the deviation of the predicted static and dynamic layouts. $\mathcal{L}_{short}^{c}$ is the short-range consistency loss and  $\mathcal{L}_{long}^{c}$ is the long-range consistency loss. $\lambda_{sup}$, $\lambda_{short}^c$ and $\lambda_{long}^c$ are the weights corresponding to the supervised, short-range consistency and long-range consistency losses respectively. Finally, $\mathcal{L}$ is the total weighted loss used for backpropagating gradients through the network. \footnote{$\lambda_{sup} > \lambda_{short}^{c} >> \lambda_{long}^c$}. Consistency loss acts as a soft constraint on the layout prediction objective $\mathcal{L}_{sup}$, which enables the model to learn more temporally consistent layout. 



% ($\mathcal{S}_{\phi, \nu}(\mathcal{I}^^i)$, $\mathcal{D}_{\phi, \nu}(\mathcal{I}^^i)$) with their corresponding ground-truth values ($\mathcal{S}^i_{gt}$, $\mathcal{D}^i_{gt}$). The adversarial loss $\mathcal{L}_{adv}$ encourages the distribution of layout estimates from the static/dynamic scene decoders ($p_{fake}$) to be close to their true counterparts ($p_{true})$. The discriminator loss $\mathcal{L}_{discr}$ is the discriminator update objective \cite{GAN}.


% \begin{figure*}[!h]
%   \centering
% %   \vspace{-3.5cm}
%   \includegraphics[width=0.9\linewidth]{figures/architecture.png}
% %   \vspace{-3.5cm}
%   \caption{\textbf{Lane Layout Estimation}: }
%   \label{fig: main_architecture}
% \end{figure*}


\subsection{Refinement Network}

% The layouts estimated by the static and dynamic decoders are sent to a Binary GAN for refinement. 

Similar to \cite{monolayout}, we use adversarial regularization in order to restrict the encoder-decoder network into predicting conceivable layouts. For adversarial regularization, we use a Patch Discriminator which takes the output of the encoder-decoder and a sample from the true data distribution. Unlike \cite{monolayout}, we make use of ground-truth layouts to do paired training with the discriminator which further improves the performance of the model. Adding the sampling layer in the static decoder converts the Encoder-Decoder network into a generator and further helps in regularization for static layouts.






% Unlike \cite{monolayout}, which uses two discriminators to directly regularize the predicted layouts from the static and dynamic decoders, we use a single refinement network to post-process the predicted layouts in order to be consistent with a prior data distribution of conceivable scene layouts. The prior data distribution is a collection of annotated lanes, vehicles and road layouts from the \autolay{} and Argoverse\cite{chang2019argoverse} dataset. 

% We use a conditional GAN similar to the Pix2Pix\cite{pix2pix} architecture as our refinement network. The neurons of the output layer of the generator are replaced with binary neurons, which restricts the generator to predict only binary maps. Outputs from the static and dynamic decoders are combined together to make a $D*D*k$ representation $\mathcal{O}$ where each pixel corresponds to a k-dimensional vector corresponding to k output classes(lanes, vehicle and road). This k-dimensional representation is then sent to the generator which outputs a refined layout $\mathcal{\hat{O}}$ in order to match the true data distribution. A patch disriminator is used to classify whether the generated layout $\mathcal{\hat{O}}$ as true or fake.

% \vspace{-1em}
% \begin{align*}
%     \mathcal{L}_g = \sum_{i=1}^{k}  \| \mathcal{O} - \mathcal{\hat{O}} \|^2 + \lambda_{adv}* \mathbb{E}_{\theta \sim p_{fake}}\left[(D(\mathcal{\hat{O}}) - 1)^2\right] \\
%     \mathcal{L}_{d} = \mathbb{E}_{\theta \sim p_{true}}\left[(D(\hat{O}) - 1)^2\right] + \mathbb{E}_{\theta \sim p_{fake}}\left[(D(\hat{O}) - 1)^2\right]    
% \end{align*}

% Loss functions $\mathcal{L}_g$ and $\mathcal{L}_{disc}$ are used for updating the parameters of the refinement GAN. $\lambda_{adv}$ is the tradeoff parameter between the pixel-wise loss between the input layout $\mathcal{O}$ and the refined output $\mathcal{\hat{O}}$ and the adversarial loss. 



% \begin{equation}
%     \begin{gathered}
%         \mathcal{L}_{adv}(L; \phi, \theta, \psi) = \mathbb{E}_{\theta \sim p_{fake}}\left[(D(\theta) - 1)^2\right]  \\
%         \mathcal{L}_{discr}(D; \theta) = \sum_{\theta \in \{\theta_D, \theta_S\}} \mathbb{E}_{\theta \sim p_{true}}\left[(D(\theta) - 1)^2\right] +\\ \mathbb{E}_{\theta \sim p_{fake}}\left[(D(\theta) - 1)^2\right]
%     \end{gathered}
% \end{equation}




% \begin{align*}
%         \mathcal{L}_{adv}(L; \phi, \theta, \psi) = \mathbb{E}_{\theta \sim p_{fake}}\left[(D(\theta) - 1)^2\right]  \\
% \end{align*}
% \vspace{-2cm}
% \begin{align*}
%         \mathcal{L}_{discr}(D; \theta) = \sum_{\theta \in \{\theta_D, \theta_S\}} \mathbb{E}_{\theta \sim p_{true}}\left[(D(\theta) - 1)^2\right] +\\ \mathbb{E}_{\theta \sim p_{fake}}\left[(D(\theta) - 1)^2\right]
% \end{align*}

% Instead of regularizing the decoders directly to produce outputs which match a prior data distribution of conceivable scene layout, we use Binary GAN as a refinement layer to post-process the outputs generated by the static and dynamic decoders .

% To better ground the likelihoods $P(\mathcal{S}|\mathcal{C}, \mathcal{I})$, $P(\mathcal{D}|\mathcal{C}, \mathcal{I})$ (\cf Eq.~\ref{eqn:map-estimation}), we introduce adversarial regularizers (discriminators) parameterized by $\theta_S$ and $\theta_D$ respectively. The layouts estimated by the static and dynamic decoders are input to these patch-based discriminators\cite{isola2017image}. The discriminators regularize the distribution of the output layouts (\emph{fake data} distribution, in GAN \cite{GAN} parlance) to match a prior data distribution of \emph{conceivable} scene layouts (\emph{true data} distribution). This prior data distribution is a collection of road snippets from OpenStreetMap \cite{OpenStreetMap}, and rasterized images of vehicles in \bev{}. Instead of training with a paired OSM for each image, we choose to collect a set of diverse OSM maps representing the true data distribution of road layouts in \bev{} and train our discriminators in an unpaired fashion. This mitigates the need to have perfectly aligned OSM views to the current image, making \monolayout{} favourable compared to approaches like \cite{schulter2018learning} that perform an explicit alignment of the OSM before beginning processing.



\subsection{Data Preparation: Weak Supervision}
\label{seubsec:dataprep}

Since the amodal scene layout labels are not provided for almost every autonomous driving dataset, we propose a generic layout generation method to generate noisy or weak supervision layout labels for static classes like roads, lanes, and sidewalks (\cf{}~Fig.~\ref{fig: weak_supervision}). Our weak supervision layout generation method is similar to the sensor fusion approach adopted in \cite{monolayout}. Further, we provide a solution to obtain weak supervision layout labels for lanes as well. 

The process of aggregating / registering the lidar points for several image frames and projecting them to an orthographic view by assuming a flat plane is shown in Fig.~\ref{fig: weak_supervision}. To obtain lanes, we perform the registering process for road and lane marker semantic classes. We then obtain lane boundary curves by isolating individual lane boundaries through Density Based Spatial Clustering and fit third order polynomial curves on these individual lane boundaries. From the registered road layout, we estimate the road boundaries and group the road and lane boundaries together to obtain lane contours.

Additionally, we also obtain improved weak supervision layout for roads by addressing cases where there are too many stationary obstacles in a sequence occluding lidar from capturing the road layout. We register lidar points belonging to those stationary obstacles that lie on the road.  

%Given a sequence, we identify which points in the corresponding lidar scan of an rgb frame belongs to a particular class (road / sidewalk / lane marking), using either the available ground truth semantic segmentation labels or labels generated using a state-of-the-art semantic segmentation network. Using the odometry information, we register these per frame class specific point clouds to obtain a dense representation of that particular class for the sequence. While registering these per frame class specific point clouds, we remove points which are more than 30 meters away from the ego-vehicle, to account for noises in semantic segmentation. These dense point clouds are then projected to every camera coordinate frame and by following a flat-plane assumption, we obtain an occupancy grid in the bird's eye view. Each cell in the occupancy grid is assigned the class label of the majority class points that fall within the cell. Unlike [] where the registration is performed with a fixed window of frames, registering the point clouds for the entire sequence also ensures a smooth layout in complex urban scenarios where the ego-vehicle is stationary for a considerable number of frames. 

%This method fails to provide the amodal layout labels for roads and sidewalks in presence of static objects like parked or stationary vehicles, which is the case in many residential or highway scenes. We address this issue by identifying if the static objects are present on these classes. This is done by considering small regions of confidence around the corners of the objects' 3D bounding boxes. These boxes are then projected to the occupancy grid with the majority class label of the dense point clouds within the regions of confidence. 

%To obtain different lane segments in the road occupancy grid, similar registration is performed for lane marker class. By using clustering and polynomial fitting, we obtain different lane boundary curves which divide the road occupancy grid into different lane segments.  
 % \documentclass{article}
% \usepackage[utf8]{inputenc}

% \setlength{\arrayrulewidth}{1mm}
% \setlength{\tabcolsep}{18pt}
% \renewcommand{\arraystretch}{1.5}

% \begin{document}
% \begin{tabular}{ |p{3cm}|p{3cm}|p{3cm}|p{3cm}|p{3cm}|p{3cm}  }
% \hline
% \multicolumn{3}{|c|}{Country List}
% \multicolumn{3}{|c|}{Country List} \\
% \hline
% Country Name     or Area Name& ISO ALPHA 2 Code &ISO ALPHA 3 Country Name     or Area Name& ISO ALPHA 2 Code &ISO ALPHA 3 \\

% \hline
% Afghanistan & AF &AFG \\
% Aland Islands & AX   & ALA \\
% Albania &AL & ALB \\
% Algeria    &DZ & DZA \\
% American Samoa & AS & ASM \\
% Andorra & AD & AND   \\
% Angola & AO & AGO \\
% \hline
% \end{tabular}
% \end{document}

==> autolay-iros-2020 (1)/text/dataset.tex <==
\section{AutoLay Dataset}



Over the last decade, several public datasets~\cite{KITTI, oxfordrobotcar, nuscenes2019, apolloscape, chang2019argoverse} have enabled massive strides in autonomous driving research. While nearly all the above datasets provide out-of-the-box support (annotations, evaluation utilities, metrics, benchmarking support) for popular tasks like object detection, semantic segmentation, multi-object tracking, trajectory forecasting, none of these currently benchmark amodal scene layout estimation.

Obtaining training data for the task of amodal layout estimation involves multiple challenges. It involves perceiving scene segments that are not even imaged by the camera. 
While most datasets have lidar scans that often span a larger sensor swath, such lidar beams are not dense enough to perceive thin scene structures.
Approaches such as \monolayout{}~\cite{monolayout} compensate for this lack of precision training data by adversarial learning, using OpenStreetMap~\cite{OpenStreetMap} data.
More recently, Wang \etal~\cite{wang2019parametric} release a dataset that provides a \emph{parametric} \bev{} representation for images from the KITTI~\cite{KITTI} and nuScenes~\cite{nuscenes2019} datasets, but the top-view representations are synthesized views of a simulated parametric surface model. In summary, there is currently no dataset that provides off-the-shelf support for benchmarking amodal layout estimation. We fill this void with \coolname, a dataset for amodal layout estimation in \bev{} (Fig.~\ref{fig:teaser_new}).

\subsection{Dataset overview}

We use $44$ video sequences from the KITTI Raw dataset~\cite{KITTI} in \coolname. We provide per-frame annotations in perspective, orthographic (\bev), as well as in 3D. Of the $44$ annotated sequences, $24$ sequences---containing $10705$ images---are used for training. The other $20$ sequences---comprising $5626$ images---form the test set. This makes for nearly $16$K annotated images, across a distance of $12$ Km, and a variety of urban scenarios (\emph{residential}, \emph{city}, \emph{road}) (\cf~Fig~\ref{fig:dataset}).
The semantic classes considered in this dataset are \emph{road}, \emph{sidewalk}, \emph{vehicle}, \emph{crosswalk}, and \emph{lane}.
Each \emph{lane} segment is provided a unique id, which we classify further\footnote{We perform this subclassification for our specific task, by projecting lane segments to \bev.}
The \emph{lane} class is further classified as \emph{ego-lane} and \emph{other lane}. We also have an \emph{other road} class for road areas that do not fall under any of the above categories.


\subsection{Data annotation}

Since annotating amodal layout from a single image is a hard task even for professional annotators, we leverage multiple sources of information to guide this procedure. We first build a point cloud map of the entire scene, annotate the map (in full 3D), and then generate the other views (\bev{}).
To build a map of the entire area, we use the lidar scans corresponding to each frame and register them to a global view. We use the precise odometry information provided in KITTI for registration, to be robust to outliers, as many scenes contain dynamic objects (vehicles/pedestrians).
To reduce manual effort, we semi-automate the data annotation pipeline to the extent possible. As a first step, we identify lane markers by choosing a range of remission values of the lidar and thresholding the 3D map.
Once a set of lane markers are identified, we tag as \emph{lanes} the area between pairs of lane markers. Manual verification is performed to ensure no discrepancies creep in.
Each identified \emph{lane} is labeled with a different \emph{lane id}, unique within a given sequence.
Annotators are then presented with this preprocessed map in an orthographic view and asked to amodally complete annotations. Specifically, chunks of missing points in a lane are \emph{filled in} as \emph{lanes}, and so on. Other identified chunks are annotated as \emph{sidewalk}, \emph{crosswalk}, or \emph{other road}. We repurpose the annotation tool from Semantic KITTI~\cite{semantickitti} for this.

Note that the above annotation procedure can only be used for static parts of the scene. For dynamic scene components, such as vehicles, a 3D bounding box annotation is performed per-frame. This entire annotated sequence is then projected into \bev{} and semantics are made available in every camera frame in the sequence. 

% \Madhav{Jump in the flow here. How does the previous statement relate to the next }

% % dataset annotation method
% \begin{itemize}
%     \item The lidar point cloud registered for an entire sequence is annotated at first. Lane blocks are identified using the difference in remission value for lidar points belonging to roads and lane markers. 
%     \item Each lane block is given a different lane id. Sidewalks and crosswalks are marked with the same id throughout the annotation process. 
%     \Madhav{Some of these can be better explained with Figs. Such as what is a lane bloc is unclear for me just by reading text}
%     \item The lidar annotation is done in an othographic view, where even points belonging to vehicles lying on a lane block are labeled with the corresponding lane id. This annotation is done using the same tool as semantic kitti  
%     \item The vehicles are annotated as 3D bounding boxes. 
%     \item The annotated point cloud is then projected in Bird's Eye View corresponding to every camera frame in a sequence with a flat plane assumption. The lidar points are projected to an occupancy grid of resolution 9mm * 9mm. 
%     \item To account for sparsity in case of static ego vehicle and sparsity at the begining and end of the sequences, we obtain a bounding box around each lane block in Bird's Eye View  \todo{THis is super-unclear to me}
% \end{itemize}

% % dataset statistics
% \begin{itemize}
%     \item There are totally 32 sequences, which are split into 16 training and 16 testing sequences. 
%     \item The training set has a total of 6608 frames. The testing set has a total of 5244 frames.
%     \item The 32 sequences are divided on the basis of number of residential, city and road sequences. 
%     \item The lane blocks in every sequence can be post processed according to the convention we require, to order lanes. 
%     \item We have also provided modified lane blocks where only lanes belonging to the road in which the ego vehicle is currently present are numbered and rest of the lane blocks are classified as other roads. 
%     \item The statistics for the total number of frames with sidewalks, crosswalks and specified number of lanes are provided. We have also provided the total number of frames annotated in every category (residential, city and road)
% \end{itemize}

==> autolay-iros-2020 (1)/text/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

% \epigraph{Imagination is `a necessary ingredient of perception itself'}{Strawson, 1974.}
% \Madhav{Why is there an epigraph? Let us not become too cute and rub folks the wrong way}
    
Commercial interest in autonomous driving has led to the emergence of several interesting and challenging problems, particularly in terms of perception. In this work, we focus on the problem of \emph{amodal scene layout estimation} (introduced in~\cite{monolayout}). \emph{Amodal} perception, as studied by cognitive scientists, refers to the phenomenon of ``imagining" or ``hallucinating" parts of the scene that do not result in sensory stimulation. In the context of urban driving, we formulate the \emph{amodal layout estimation} task as predicting a \bev{} semantic map from monocular images that explicitly reasons about entities in the scene that are not visible from the image(s).

Amodal scene layout estimation is an emerging area of study where prior efforts~\cite{monolayout, monooccupancy, schulter2018learning} have only focused on amodal completion for \emph{coarse} categories such as roads and sidewalks. While recent efforts have incorporated dynamic objects~\cite{monolayout}, they fall short of modeling higher-level behaviors in urban driving scenarios such as lane-keeping, merging, etc. Further, each of these efforts~\cite{monolayout, monooccupancy, schulter2018learning} lack consensus in problem specifications and evaluation protocols.
% This is in part due to the unavailability of datasets for learning rich semantic representations, and the absence of a unified evaluation protocol for prior approaches.

We address both the above issues. We first formalize the problem of \emph{amodal scene layout estimation} that unifies existing work and extends the task to several fine-grained categories. To foster research in this area, we provide \coolname{}, a dataset comprising of over $16000$ images over a distance of $12$ kilometers, annotated with fine-grained \emph{amodal} completions in 3D as well as in \bev. \coolname{} includes $44$ sequences from KITTI~\cite{KITTI} and $89$ sequences from the Argoverse~\cite{chang2019argoverse} datasets. We implement several baselines and prior art, and open-source our code, models, and data~\cite{monolayout, monooccupancy, you2019pseudo}. We additionally propose \videolayout{}, a simple approach that achieves top performance on the \coolname{} benchmark by leveraging temporal information across image sequences, advancing the state-of-the-art of amodal layout estimation.

% We further present \videolayout{}, a neural architecture for amodal scene layout estimation from monocular video. \videolayout{} achieves state-of-the-art performance on the \coolname{} benchmark, and produces coherent layout estimates over long image sequences. We open-source all our implementations and pretrained models, for reproducibility.\footnote{Code and dataset to be released upon acceptance. For examination purposes, samples from the dataset are provided on our project page: \url{https://hbutsuak95.github.io/AutoLay/}}


% \Krishna{Intentionally skipping explicit contribution list. I think we have a strong case in the remainder of the paper.}

% \Madhav{In this fast world everyone wants to have a digest version of the paper. Many may want a quick idea of what the paper contributes and read the paper from thereoff. }



\begin{figure*}[!ht]
  \centering
  \includegraphics[width=\textwidth]{images/autolay_dataset_statistics.png}
  \captionof{figure}{\textbf{Dataset}: (\emph{Left to right}) Sample images from the \emph{KITTI} split of \coolname{}. Corresponding annotated lidar pointclouds. Amodal scene layout in \bev{}. (\emph{Last column}) Distribution of semantic classes (bar plot), and scene types (pie chart).
}
  \label{fig:dataset}
\end{figure*}

% As opposed to current art~\cite{monolayout, monooccupancy, schulter2018learning}, which focuses on coarse-classes such as roads/sidewalks, we include fine-grained categories such as lanes, crossroads, etc. that play a crucial role in understanding the semantics of road scenes.

% The key contributions of our work are as follows:

% \begin{compactenum} 
%     \item We release KITTI-Layout dataset which provides annotated groundtruth layouts in bird's eye view for traffic participants like lanes, vehicles, sidewalks, etc. 
    
%     \item We also release precise point-cloud annotations for over 40 KITTI sequences in Lidar space. 
    
%     \item We provide evaluation of several state-of-the-art layout prediction methods on the KITTI-Layout dataset. 
    
%     \item Furthermore, we propose an extension to MonoLayout in order to incorporate temporal information which in turn helps in generating temporally consistent layouts.  
    
%     \item The proposed method outperforms all of the several state-of-the-art approaches by a significant margin on a number of datasets(KITTI-Layout, KITTI-Raw \cite{schulter2018learning}, Argoverse \cite{chang2019argoverse}).
    
    
% \end{compactenum}

==> autolay-iros-2020 (1)/text/problem.tex <==
\section{Amodal scene layout estimation}
\label{sec:problem}






We begin by formally defining the task of amodal scene layout estimation. Given an image (or a sequence of images) $\mcal{I}$, usually in perspective view, we wish to learn a \emph{labeling function} $\Phi$ of \emph{all} points within an area $\mcal{R}$ (usually rectangular) around the camera. The region of interest $\mcal{R}$ is often in a different view than that of the perspective image. In this paper, we focus on \bev{}, which refers to a top-down orthographic view of the ground plane. The labeling function $\Phi$ must produce a label distribution (over a set of $N$ classes) for world points within the swath $\mcal{R}$, \emph{regardless of whether or not they are imaged in} $\mcal{I}$.

In particular, we propose the estimation of the following semantic classes tasks in the context of this problem: road, sidewalk, crosswalk, lanes (ego-lane, other lanes), other road, vehicle. Depending on the exact setup used (single-image vs image-sequences, semantic categories to be estimated, etc.), this enables fair evaluation of all approaches. We defer a detailed description of evaluation protocols and its challenges to Sec.~\ref{sec:experiments}.
% each approach must be evaluated against others on equal footing.

% \Kaustubh{
% Tasks we've proposed for achieving amodal scene layout estimation are:

% \begin{itemize}
%     \item Road Layout Detection 
%     \item Vehicle Layout Estimation 
%     \item Ego-Lane estimation 
%     \item Overall Lane estimation 
% \end{itemize}

% }


==> autolay-iros-2020 (1)/text/relatedwork.tex <==
\section{Related work}
\label{sec:relatedwork}


% \begin{figure}[!t]
%   \centering
%     \begin{adjustbox}{max width=0.8\linewidth}
%     \includegraphics[]{figures/lanes_plot.jpg}
%     \end{adjustbox}
% \end{figure}

Interpreting 3D scenes from an RGB image has been a longstanding challenge for computer vision systems. In this section, we enlist a few approaches to \emph{amodal} perception. For a comprehensive survey of general 3D scene understanding, we refer the interested reader to Ozyecsil \etal~\cite{ozyecsil2017survey}.

\subsubsection*{\textbf{Amodal perception for indoor scene understanding}}

% With the advent of deep learning, substantial progress has been made in estimating scene semantics from a single image~\cite{saxena2008make3d, wu2016learning}. However, most such approaches only reason about objects/regions visible in an image.
In the context of indoor 3D scene understanding, a few approaches to \emph{amodal} perception have been proposed~\cite{amodalKTCM15, factored3dTulsiani17}. While these approaches use coarse voxel grids to represent objects, we instead focus on an orthographic top-down view that restricts semantic understanding to road regions. We note that most of the semantic understanding necessary for driving-related tasks can be obtained on the road regions, making this simplification attractive.
% \cite{factored3dTulsiani17} attempts to estimate the 3D scene layout from a single RGB image of indoor scenes and represents object using a coarse voxel grid. In this work, however, we focus on an orthographic top-down view as such a view can potentially subsume most of the semantic information necessary for scene understanding in urban driving settings.
% However, in this work, we aim to predict an occlusion aware amodal scene layout estimation of static (roads, sidewalks, lanes) and dynamic (vehicles) classes in outdoor scenes. 

% \subsubsection*{\textbf{Amodal perception in perspective view}}

% % There have been attempts in the past towards amodal perception from an RGB image. 
% % , benchmarked on datasets like \cite{KITTI} and \cite{cordts2016cityscapes}. But these works were not focussed on reasoning occluded regions in perspective view. 
% % As an example, consider the task of inpainting foreground objects.
% % foreground objects in perspective view can help in understanding occluded regions. 
% % Pathak \etal~\cite{pathak2016context} developed Context Encoders which use other parts of an image to predict missing patches from an image. Uittenbogaard \etal~\cite{uittenbogaard2019privacy} propose a moving object segmentation method that inpaints regions using images from other views.
% A few recent approaches~\cite{schulter2018learning, lu2020semantic} explicitly reason about occluded image pixels by inpainting foreground objects with semantic labels of background classes and estimating their per-pixel depth.
% In this work, we focus on \bev{} and amodal perception therein.

% \subsubsection*{\textbf{Layout estimation in Bird's Eye View}}

\subsubsection*{\textbf{Amodal perception for autonomous driving}}

To the best of our knowledge, there are no previous works that provide a unified approach to obtain an amodal scene layout estimation in \bev{} for fine-grained static and dynamic classes like lanes, sidewalks, vehicles, etc. Existing approaches~\cite{monooccupancy, schulter2018learning, wang2019parametric, lu2019hallucinating} reason about ``coarse-grained" static classes such as roads and sidewalks. Schulter \etal~\cite{schulter2018learning} obtain occlusion-aware \bev{} road layouts by hallucinating behind objects tagged as \emph{foreground} in an image.
% The layout structures were refined through adversarial learning using road shapes from Open Street Maps \cite{OpenStreetMap}.
Wang \etal~\cite{wang2019parametric} develop a parametric representation of road scenes that reason about the number of lanes, width of each lane, presence of an intersection, etc.
Lu \etal~\cite{monooccupancy} use a variational autoencoder to predict road, sidewalk, terrain, and non free-space in bird's eye view.
% However, they perform layout estimation only in the image field of view. Similar to \cite{schulter2018learning}, \cite{lu2019hallucinating} rely on \cite{OpenStreetMap} and semantic class impainting to obtain the road layout. 
Lu~\etal{}~\cite{lu2019hallucinating} also perform vehicle shape completion, albeit independent of the static layout estimation task.
Garnett~\etal{}~\cite{garnett20193d} predict static road and lane layouts by estimating lane boundaries in 3D.

For dynamic scene understanding, several approaches aim to detect object layouts in 3D. While some of these~\cite{ku2018joint, chen2017multi, liang2018deep} combine information from images and lidar, others~\cite{yang2018pixor, roddick2018orthographic, wang2019pseudo} operate by converting images to \bev{} representations, followed by object detection. However, these techniques are often developed independently of static layout estimation methods.

In earlier work, we presented MonoLayout~\cite{monolayout}- perhaps the first approach to amodally reason about the static and dynamic layout of an urban driving scene. While the interest in this nascent area is rapidly increasing, the absence of standardized task specification and evaluation have been slowing down research. This forms the primary motivation behind the \coolname{} dataset and benchmark.

% Similarly, several existing approaches for vehicle layouts in bird's eye view are based on 3D object detection. These approaches can be broadly classified into raw point cloud based or grid/voxel based object detection. \cite{yang2018pixor} converts the lidar point cloud to a grid representation in bird's eye view to process for object detection. \cite{ku2018joint}, \cite{chen2017multi} and \cite{liang2018deep} focus on combining information from lidar and RGB images for object detection. \cite{shi2019pointrcnn} uses raw lidar point cloud to get object region proposals which are then refined to generate 3D bounding boxes. \cite{roddick2018orthographic} developed Orthographic Feature Transform to map extracted features from an RGB image to the corresponding bird's eye view. \cite{wang2019pseudo} and \cite{you2019pseudo} make use of depth estimation networks from RGB images to obtain a dense point cloud on which \cite{ku2018joint} is used for object detection.  
 
% In summary, we present the first approach---to the best of our knowledge---to estimate amodal layout for fine-grained classes from a single image. We also extend the approach to handle multiple images and predict temporally coherent layout estimates.

%On the other hand, we propose \emph{VideoLayout} in similar lines to \emph{Monolayout}, where we provide temporally consistent amodal scene layout in bird's eye view for road, vehicle and lane classes, given a sequence of  





==> autolay-iros-2020 (1)/text/results.tex <==
\section{Experiments}
% \label{sec:experiments}
% \begin{table*}[!ht]
% \begin{center}
% \begin{adjustbox}{max width=\linewidth, totalheight=3.5cm}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \centering

% % \toprule
%                             & \multicolumn{2}{c|}{Vehicle Layout}                     & \multicolumn{6}{c|}{Static Layout Estimation}       \\ \hline 
%                             &           &                                                & \multicolumn{2}{c|}{Road}   & \multicolumn{4}{c|}{Lane}  \\  \cline{4-9} 
%           Method            &           &                   &             &             &  \multicolumn{2}{c|}{Ego-Lane}    &      \multicolumn{2}{c|}{OverAll}   \\ \cline{6-9}
%                                               & mIoU      &     mAP           &  mIoU       & mAP         &   mIOU    &   mAP   &      \small{$AP_{IOU>0.7}$}   &   \small{$Recall_{IOU>0.7}$}   \\
%                                                     \cline{1-9} 
% MonoOccupancy-ext           & $16.41$   &      $21.06$      & $67.66$     &  $74.73$    &   $63.77$   & $74.49$   &     $22.04$   &  $24.82$     \\
%  PseudoLidar-ENet           & $21.12$   &      $31.19$      & $61.22$     &  $68,72$    &   $53.11$   & $65.90$   &     $8.79$    &  $6.44$             \\
%  PseudoLidar-UNet           & $24.37$   &      $38.08$      & $64.41$     &  $70.23$    &   $55.81$   & $66.03$   &     $11.74$   &  $9.76$      \\
%  MonoLayout\cite{monolayout}& $21.05$   &      $32.42$      & $69.72$     &  $82.22$    &   $65.46$   & $78.48$   &     $27.88$   &  $25.89$       \\                                                     
%  VideoLayout                & $\mb{25.47}$   &      $\mb{39.67}$      & $\mb{76.49}$     &  $\mb{87.62}$    &   $\mb{71.07}$   & $\mb{83.49}$   &     $\mb{50.15}$   &  $\mb{34.95}$      \\      
% \hline
% \end{tabular}
% \end{adjustbox} 
% \end{center}
% \caption{\textbf{Quantitative results}:
% We benchmark \videolayout{}, \monolayout{} \cite{monolayout}, MonoOccupancy \cite{monooccupancy} and PseudoLidar based approaches on \coolname{}. The evaluation metric scores are reported for various methods with weak(\cf{} Sec.~\ref{seubsec:dataprep}) and strong(annotated ground truth labels) supervision for static layout estimation and only wi
% th strong supervision for vehicle layout estimation.}
% \label{table:quantitative:main}
% \end{table*}


% \Madhav{Very important to cite Mono Layout in the Tables and any such prior work. }

% \begin{figure*}[!t]
%     \centering
%     \begin{adjustbox}{max width=0.9\linewidth, totalheight=13cm}
%     \begin{tabular}{ccc|ccc}
%         \toprule
%         \multicolumn{3}{c|}{KITTI}     &   \multicolumn{3}{c}{Argoverse} \\
%         % \hline 
%         \midrule
%         \frame{\includegraphics[width=30mm,height=20mm]{images/rgb/0000000062.png}}
%         & \frame{\includegraphics[width=20mm,height=20mm]{images/pred/0000000062.png}}
%         & \frame{\includegraphics[width=20mm,height=20mm]{images/gt/0000000062.png}}
%         & \frame{\includegraphics[width=30mm,height=20mm]{images/rgb/stereo_front_left_315980123132577904.jpg}}
%         & \frame{\includegraphics[width=20mm,height=20mm]{images/pred/stereo_front_left_315980123132577904.png}}
%         & \frame{\includegraphics[width=20mm,height=20mm]{images/gt/stereo_front_left_315980123132577904.png}} \\
        
%         \frame{\includegraphics[width=30mm,height=20mm]{images/rgb/0000000089.png}}
%         & \frame{\includegraphics[width=20mm,height=20mm]{images/pred/0000000089.png}}
%         & \frame{\includegraphics[width=20mm,height=20mm]{images/gt/0000000089.png}}
%         & \frame{\includegraphics[width=30mm,height=20mm]{images/rgb/stereo_front_left_315976463818684936.jpg}}
%         & \frame{\includegraphics[width=20mm,height=20mm]{images/pred/stereo_front_left_315976463818684936.png}}
%         & \frame{\includegraphics[width=20mm,height=20mm]{images/gt/stereo_front_left_315976463818684936.png}} \\
         
%         \frame{\includegraphics[width=30mm,height=20mm]{images/rgb/0000000319.png}}
%         & \frame{\includegraphics[width=20mm,height=20mm]{images/pred/0000000319.png}}
%         & \frame{\includegraphics[width=20mm,height=20mm]{images/gt/0000000319.png}}
%         & \frame{\includegraphics[width=30mm,height=20mm]{images/rgb/stereo_front_left_315980120734975008.jpg}}
%         & \frame{\includegraphics[width=20mm,height=20mm]{images/pred/stereo_front_left_315980120734975008.png}}
%         & \frame{\includegraphics[width=20mm,height=20mm]{images/gt/stereo_front_left_315980120734975008.png}} \\
        
%         \frame{\includegraphics[width=30mm,height=20mm]{images/rgb/0000000018.png}}
%         & \frame{\includegraphics[width=20mm,height=20mm]{images/pred/0000000018.png}}
%         & \frame{\includegraphics[width=20mm,height=20mm]{images/gt/0000000018.png}}
%         & \frame{\includegraphics[width=30mm,height=20mm]{images/rgb/stereo_front_left_315966714192012400.jpg}}
%         & \frame{\includegraphics[width=20mm,height=20mm]{images/pred/stereo_front_left_315966714192012400.png}}
%         & \frame{\includegraphics[width=20mm,height=20mm]{images/gt/stereo_front_left_315966714192012400.png}} \\
        
%         \frame{\includegraphics[width=30mm,height=20mm]{images/rgb/0000000298.png}}
%         & \frame{\includegraphics[width=20mm,height=20mm]{images/pred/0000000298.png}}
%         & \frame{\includegraphics[width=20mm,height=20mm]{images/gt/0000000298.png}}
%         & \frame{\includegraphics[width=30mm,height=20mm]{images/rgb/stereo_front_left_315968399894870816.jpg}}
%         & \frame{\includegraphics[width=20mm,height=20mm]{images/pred/stereo_front_left_315968399894870816.png}}
%         & \frame{\includegraphics[width=20mm,height=20mm]{images/gt/stereo_front_left_315968399894870816.png}} \\
        
%         % \frame{\includegraphics[width=30mm,height=20mm]{images/vehicles/003194.png}}
%         % & \frame{\includegraphics[width=20mm,height=20mm]{images/vehicles/003194_monoocc.png}}
%         % & \frame{\includegraphics[width=20mm,height=20mm]{images/vehicles/003194_mono3d.png}}
%         % & \frame{\includegraphics[width=20mm,height=20mm]{images/vehicles/003194_oft.png}}
%         % & \frame{\includegraphics[width=20mm,height=20mm]{images/vehicles/003194_monolayout.png}}
%         % & \frame{\includegraphics[width=20mm,height=20mm]{images/vehicles/003194_gt.png}} \\
%         \midrule
%         RGB & \videolayout{} & \textit{GroundTruth} & RGB & \videolayout{} & \textit{GroundTruth} \\
        
%         \bottomrule
%         % \textbf{RGB} & \textbf{Lu et al.\cite{lu2019monocular}} & \textbf{Mono3D\cite{chen2016monocular}} & \textbf{OFT\cite{roddick2018orthographic}} & \textbf{Ours} & \textbf{GT}
        
%     \end{tabular}
%     \end{adjustbox}
%     \caption{\footnotesize{\textbf{Static layout estimation}: \videolayout{} predicts fine-grained attributes of the road scene including lanes, side roads and ego-lane. Each individual color represents a single lane. Ego-lane is shown in {\textcolor{blue}{blue}} and side-roads are shown in  light  {\textcolor{orange}{orange}}. \videolayout{} produces decent static layout estimates for both AutoLay and Argoverse datasets. Its able to hallucinate occuled regions in the scene very reliably specially for Argoverse dataset.}}
%     % \Kaustubh{Row1: Occlusion Awareness/Amodal Completion, Row2: No occlusion, Row3 and Row4: Hallucination Power and Challenging scenarios, Row5: ARGO results}
%     \label{fig:qualitative_road}
%     \vspace{-0.5cm}
% \end{figure*}

\begin{figure*}[!ht]
  \centering
    \begin{adjustbox}{max width=0.9\linewidth, totalheight=13cm}  \includegraphics[width=0.8\linewidth]{images/autolay_static_results.png}
    \end{adjustbox}
    \caption{\footnotesize{\textbf{Static layout estimation}: \videolayout{} predicts fine-grained attributes of the road scene including lanes, side roads and ego-lane. Each individual color represents a single lane. Ego-lane is shown in {\textcolor{blue}{blue}} and side-roads are shown in  light  {\textcolor{orange}{orange}}. \videolayout{} produces decent static layout estimates for both AutoLay and Argoverse datasets. Its able to hallucinate occluded regions in the scene very reliably specially for Argoverse dataset.}}
  \label{fig:qualitative_road}
  \vspace{-0.5cm}
\end{figure*}





% \begin{table}[]
%     \centering
%     \begin{adjustbox}{max width=\textwidth, totalheight=1.7cm}
%     \begin{tabular}{|c|c|c|c|c|c|}
%         \hline
%                         & \multicolumn{2}{c|}{Vehicle}     & Road        & \multicolumn{2}{c|}{Lane}       \\
%         \cline{2-6}
%         Method                        & mIOU        &  mAP               & mIOU        & Ego-Lane  &  Overall   \\
%         \hline
%         MonoLayout(w/o sampling)      & 56.16       &  18.18             &   28.24     &  -              &  -          \\
%         MonoLayout(w/ sampling)       & 56.16       &  18.18             &   28.24     &  -              &  -          \\
%         VideoLayout(w/o sampling)     & -           &  -                 &    -        &  -              &  -  \\
%         VideoLayout(w/ sampling)      & -           &  -                 &    -        &  -              &  -  \\
%         \hline
%     \end{tabular}
%     \end{adjustbox}
%     \caption{Ablation Study: Effect of incorporating temporal information and using sampling layer in the static decoder on the performance of \monolayout{} and \videolayout{} on AutoLay dataset. }
%     \label{table:ablation}
% \end{table}


So far, there has been a lack of consensus on datasets and evaluation protocol for amodal layout estimation. We describe the \coolname{} evaluation protocol in detail, and evaluate baselines and existing approaches on the benchmark.


\subsection{Datasets}


% Till now, all the work in outdoor layout estimation has been evaluated on different datasets or on different train/test splits. We provide a detailed benchmark of the existing state-of-the-art methods for monocular layout estimation on the \autolay{} dataset. 

To ensure fair comparison with existing methods, we show our results on the Argoverse~\cite{chang2019argoverse} and KITTI RAW split used in~\cite{monolayout} and~\cite{schulter2018learning} respectively. Argoverse~\cite{chang2019argoverse} provides detailed high-resolution semantic maps in \bev{} for roads, vehicles and lanes, which makes it suitable for evaluation on all the tasks proposed in Sec.~\ref{sec:problem}. We present a breakdown of the \coolname{} benchmark below.


\begin{enumerate}
    \item \textbf{\emph{KITTI} split}: The \emph{KITTI} split of \autolay{} comprises $10705$ train images and $5626$ test images. We report results for models trained using weak (proposed data preparation) and strong (ground-truth) supervision.
    \item \textbf{\emph{KITTI RAW} split}: For fair evaluation with Schulter~\etal{}~\cite{schulter2018learning}, we use the KITTI RAW split comprising $16269$ train images and $2305$ test images).
    \item \textbf{\emph{Argoverse} split}: The Argoverse~\cite{chang2019argoverse} split contains $6722$ train images and $2418$ test images.
\end{enumerate}



% \vspace{-1cm}
\subsection{Implementation Details}


\subsubsection{PseudoLidar input}
We evaluate the performance of a set of approaches that take PseudoLidar\cite{wang2019pseudo} as input for amodal scene layout estimation. The PseudoLidar representation is a processed point cloud obtained by projecting the RGB image pixels to the camera coordinate system using the per-pixel depth values obtained from unsupervised monocular depth estimation methods like \cite{godard2018digging}. We substitute the remission value by the normalized mean of RGB channel intensities. We then obtain a voxel representation of the point cloud by slicing it vertically along the X-Z plane with a resolution of 0.15625 m and horizontally along the Y-axis into 10 channels starting from 0.4 m above the camera to 2 m below the camera. This PseudoLidar representation is provided as the input to ENet \cite{enet} or Unet \cite{unet} for amodal scene layout estimation.

\subsubsection{Lane layout convention}
In order to convert lane estimation, which is essentially an instance segmentation/detection task in \bev{} to an occupancy prediction task, we adhere to the following convention while performing lane layout estimation. While creating the per frame training labels using both weak and strong supervision, we classify the individual lane layouts on the road with the ego-vehicle, (\emph{ego-road}), as either  \emph{ego lane} or \emph{other lanes}. The ego lane and the other lanes are provided individual lane ids. The lane ids to the other lanes are given on the basis of their position with respect to the ego-lane.


% On every dataset split we evaluate on, it can be seen that the lanes lying to the right of the \emph{ego lane} are very few in number when compared to the lanes lying to the left of the \emph{ego lane}, and we accordingly penalize the cross-entropy loss for each of these other lane layouts.

\subsection{Evaluation Metrics}
 
 
 
\subsubsection{Vehicle Layout}
Similar to \cite{monolayout}, We evaluate the vehicle layouts on both mean intersection-over-union(mIoU) and mean average-precision(mAP). Since we are evaluating different methods on the task of vehicle occupancy prediction in \bev{}, we don't go for the traditional evaluation metric($AP_{IoU>0.7}$ or $AP_{IoU>0.5}$) used by 3D object detection methods or object detection methods in \bev{}. 


\subsubsection{Road Layout}

We adopt mean intersection-over-union(mIoU) and mean average-precision(mAP) as our metric for evaluating road layouts on the datasets. To evaluate hallucination capabilities of different methods, we also make use of the occluded mean intersection-over-union (IoU) used in \cite{schulter2018learning}, \cite{monolayout}. This involves calculating IoU for only the portions of the road which are occluded. 

\subsubsection{Lane Layout}
As mentioned in Sec.~\ref{sec:problem}, Lane Layouts are evaluated on two separate tasks: Ego-lane estimation and Overall lane detection. 

\begin{enumerate}
    \item \textit{Ego-Lane Estimation:} Ego-Lane estimation task is evaluated on the mean intersection-over-union (mIoU) and mean average-precision (mAP) metric.
    
    \item \textit{Overall Lane Detection:} For this task, we use $AP_{IoU>0.7}$, a popular metric used for evaluating object detection and instance segmentation methods. A predicted lane is counted as a detection if its intersection-over-union(IoU) with one of the ground truth lanes is greater than 0.7(70\%). $AP_{IoU>0.7}$ provides information about the average-precision of predicted detections. We also report $Recall_{IoU>0.7}$, which gives us an idea about the prediction capability of the method. 
\end{enumerate}

\subsection{Evaluated Methods}
We evaluate the performance of the following approaches.
\begin{itemize}
    \item \emph{Schulter~\etal{}}: The static scene layout estimation approach proposed in~\cite{schulter2018learning}.
    \item \emph{MonoOccupancy}: The static scene layout estimation approach proposed in~\cite{monooccupancy}.
    \item \emph{MonoOccupancy-ext}: We extend MonoOccupancy~\cite{monooccupancy} to predict vehicle occupancies.
    \item \emph{PseudoLidar-ENet}: A ENet~\cite{enet} architecture with PseudoLidar input for amodal scene layout estimation.
    \item \emph{PseudoLidar-UNet}: A UNet~\cite{unet} architecture with PseudoLidar input for amodal scene layout estimation.
    \item \emph{MonoLayout}: Amodal scene layout estimation architecture proposed in~\cite{monolayout}
    %\item \emph{MonoLayout-ext}: We extend the MonoLayout \cite{monolayout} to predict lane occupancies and use the data preparation method mentioned in Sec.~\ref{seubsec:dataprep} for generating weak supervision. 
    \item \videolayout: The full \videolayout{} architecture trainned with temporal-consistency loss and the adversarial refinement network.
\end{itemize}
%}
% \multirow{6}{*}{\begin{turn}{92}AutoLay \end{turn}}

\label{sec:experiments}
\begin{table*}[!ht]
\begin{center}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
\centering

% \hline
% \toprule
% \hline                                            \toprule
                                                     &                                              & \multicolumn{2}{c|}{\textbf{Vehicle Layout}} & \multicolumn{6}{c}{\textbf{Static Layout Estimation}}       \\ 
                                                    \hline
                                                     &                                              &           &                   & \multicolumn{2}{c|}{\textbf{Road}}   & \multicolumn{4}{c}{\textbf{Lane}}  \\ 
                                                    \cline{5-10} 
                                    \textbf{Dataset}          &          \textbf{Method}                              &           &                   &             &             &  \multicolumn{2}{c|}{\textbf{Ego-Lane}}    &      \multicolumn{2}{c}{\textbf{Overall}}   \\
                                                     \cline{7-10}
                                                     &                                              & \textbf{mIoU}      &     \textbf{mAP}           &  \textbf{mIoU}       & \textbf{mAP}         &   \textbf{mIoU}    &   \textbf{mAP}   &      \textbf{\small{$AP_{\small{iou>0.7}}$}}   &   \textbf{\small{$Recall_{iou>0.7}$}}   \\
                                                    \cline{1-10} 
\multirow{5}{*}{KITTI} & PseudoLidar-UNet  & $20.10$   &      $52.47$      & $57.62$     &  $70.90$    &   $51.98$  &   $68.94$   &  $8.53$ &  $19.09$         \\
                         & PseudoLidar-ENet  & $15.26$   &      $40.05$      & $55.70$     &  $67.62$    &   $54.42$  &   $68.15$   &   $13.01$   &  $24.50$     \\
                         & MonoOccupancy-ext  & $27.03$   &      $42.92$      & $63.10$     &  $77.56$    &  $58.39$  &  $69.16$   &   $26.11$   &  $35.36$         \\
             & MonoLayout\cite{monolayout}   & $30.88$   &      $53.63$      & $63.83$     &  $77.53$    &   $58.27$  &  $72.08$   &   $16.09$  &  $34.91$     \\                                                     
                                                    %  & MonoLayout-ext                               & $  -  $   &      $  -  $      & $65.58$     &  $77.37$    &   $62.26$  &  $74.90$   &     $24.12$  &  $26.11$  \\                                                     
                        & VideoLayout        & $\mb{34.60}$   & $\mb{52.87}$      & $\mb{68.73}$     &  $\mb{84.89}$    &   $\mb{62.68}$  &  $\mb{76.80}$   &     $\mb{38.56 }$  &  $\mb{44.33}$   \\                                                     
                                                    \hline
\multirow{3}{*}{Argoverse} & MonoOccupancy-ext   & $16.22$   &      $38.66$      &  $72.41$     &  $79.62$    &   $75.26$   & $85.51$   &     $39.76$   &  $51.65$     \\
                & MonoLayout\cite{monolayout}    & $28.31$   &      $46.07$      & $73.25$     &  $84.56$    &   $71.73$   & $82.00$   &     $26.18$   &  $42.61$       \\                       
                     & VideoLayout               & $\mb{32.77}$   &      $\mb{50.48}$      & $\mb{76.42}$     &  $\mb{88.01}$    &   $\mb{77.62}$   & $\mb{87.77}$   &     $\mb{46.03}$   &  $\mb{54.86}$      \\      
% \hline
\end{tabular}
\end{adjustbox} 
\end{center}
\caption{\textbf{Quantitative results}:
We benchmark \videolayout{}, \monolayout{} \cite{monolayout}, MonoOccupancy-ext and PseudoLidar based approaches on KITTI and Argoverse datasets.}
\label{table:quantitative:main}
\end{table*}


% \begin{figure*}[!ht]
%   \centering
% %   \vspace{-3.5cm}
%   \includegraphics[width=0.9\textwidth]{figures/static_layouts.png}
% %   \vspace{-3.5cm}
%   \caption{\textbf{Static Layout Estimation} Shown above are the road and lane layout estimates for few sample frames from \coolname{}. The ego lane is shown in blue. \videolayout{} predicts accurate static layouts irrespective of uneven illumination or complexity of the urban scenarios.}
%   \label{fig: static_layout}
% \end{figure*}


\begin{table}[]
    \centering
    \begin{adjustbox}{max width=\textwidth, totalheight=2.5cm}
    \begin{tabular}{|c|c|c|c|c|}
        \hline
                                                      &             &                  &  Road     &         \\

                                                      & Road        & Sidewalk         &   +      &  Lane       \\
            Method                                    &             &                  & Sidewalk &              \\
        \cline{2-5}
                                                      & mIOU        &  mIOU            &    occ mIOU     &  \small{$AP_{\small{iou>0.7}}$}  \\
        \hline
        MonoOccupancy\cite{monooccupancy}             & $56.16$       &  $18.18$       &   $28.24$       &   $26.64$          \\
        Schulter \etal{} \cite{schulter2018learning}  & $68.89$       &  $30.35$       &   $61.06$       &      -          \\
        MonoLayout\cite{monolayout}                   & $73.86$       &  $32.86$       &   $67.42$      &    $16.20$       \\
        \videolayout{}                                & $\mb{75.92}$  &  $\mb{37.74}$  &   $\mb{71.01}$  &  $\mb{36.64}$                 \\
        \hline
    \end{tabular}
    \end{adjustbox}
    \caption{State-of-the-art comparision for static layout(Road, Sidewalk and Lane) with weak supervision(\cf{} Sec. \ref{seubsec:dataprep}) on KITTI RAW split used in \cite{schulter2018learning} }
    \label{table:kittiraw}
\end{table}


% \section{Discussion}

% \begin{figure}[!t]
%     \centering
%     \begin{adjustbox}{max width=\linewidth}
%     \begin{tabular}{ccc}
%         \toprule
%         % \midrule
%         \frame{\includegraphics[width=30mm,height=20mm]{images/rgb/stereo_front_left_315968229276982120.jpg}}
%         & \frame{\includegraphics[width=20mm,height=20mm]{images/pred/stereo_front_left_315968229276982120.png}}
%         & \frame{\includegraphics[width=20mm,height=20mm]{images/gt/stereo_front_left_315968229276982120.png}} \\
        
%         \frame{\includegraphics[width=30mm,height=20mm]{images/rgb/stereo_front_left_315967482019868600.jpg}} 
%          & \frame{\includegraphics[width=20mm,height=20mm]{images/pred/stereo_front_left_315967482019868600.png}}
%          & \frame{\includegraphics[width=20mm,height=20mm]{images/gt/stereo_front_left_315967482019868600.png}} \\
         
%           \frame{\includegraphics[width=30mm,height=20mm]{images/rgb/stereo_front_left_315968412282468808.jpg}}
%          & \frame{\includegraphics[width=20mm,height=20mm]{images/pred/stereo_front_left_315968412282468808.png}}
%          & \frame{\includegraphics[width=20mm,height=20mm]{images/gt/stereo_front_left_315968412282468808.png}} \\
%         \midrule
%         RGB & \videolayout{} & \textit{GroundTruth} \\

%         \bottomrule
%         % \textbf{RGB} & \textbf{w/o Discrim.} & \textbf{With Discrim.} & \textbf{GT}
%     \end{tabular}
%     \end{adjustbox}
%     \caption{\footnotesize{\textbf{Failure Cases} of \videolayout{}. (\emph{Top row}) Failure to predict ego-lane. (\emph{Middle row}) Failure in heavy traffic scenarios. (\emph{Bottom row}) Failure in predicting lane width. 
%     % row 3 shows the case where \videolayout{} fails to predict the lane-width accurately.
%     }}
%     % \Kaustubh{add caption}
    
%     % \caption{Qualitative comparison on KITTI\cite{KITTI} for showing the effect of discriminator on road layouts. For each row, the first image is a RGB image in KITTI dataset. The second image in the row is representative of the output generated by \monolayout{} without discriminator. The third image in the row is the output generated by \monolayout{} in the presence of a discriminator. The final image in the row is the corresponding manually annotated ground truth road layout}
%     \label{fig:failure}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/dynamic_layout_argo.png}
    \caption{\textbf{Dynamic Layout Estimation:}. \videolayout{} provides crisp and accurate vehicle occupancies. The grey boxes indicate vehicle occupancies. Observe the ability of \videolayout{} to precisely localize vehicles that are distant and partially occluded. }
    \label{fig:dynamic}
\end{figure}


\subsection{Road Layout Estimation}
\label{subsec:roadlayoutest}
% We compare \videolayout{} with existing layout predictions methods like Schulter \etal{} \cite{schulter2018learning}, MonoOccupancy\cite{monooccupancy} and \monolayout{}\cite{monolayout}. We also propose two PseudoLidar based layout prediction methods 


We evaluate PseudoLidar based (PseudoLidar-UNet, PseudoLidar-ENet) and RGB image based architectures (MonoOccupancy \cite{monooccupancy}, \monolayout{} and \videolayout{}) for the task of road layout estimation using the ground truth labels. Table~\ref{table:quantitative:main} provides a detailed benchmark of these methods on the \autolay{} and Argoverse\cite{chang2019argoverse} datasets. We also perform state-of-the-art comparision(Table~\ref{table:kittiraw}) with previously proposed methods in literature on KITTI RAW split proposed in  \cite{schulter2018learning} on the task of road and lane layout estimation. For this comparision, we use the weak data generation method mentioned in Sec~\ref{seubsec:dataprep}.  

We observe that \monolayout{} and \videolayout{} perform better than PseudoLidar-based methods for road layout estimation. This can be attributed to the sparsity of the PseudoLidar points as the distance from camera increases. Also, PseudoLidar based inputs don't allow the use of deep feature encoders like ResNet\cite{he2016deep} needed to extract the rich visual features necessary for hallucinating amodal scene layouts. From Table~\ref{table:quantitative:main} it can be seen that MonoOccupancy-ext performs better than the PseudoLidar counterparts.
% \SaiShankar{There is a mention to weak supervision here}.
This further exemplifies the narrative that with better supervision, an RGB image-based architecture can reason for occluded regions better than pseudo-lidar based approaches.

Within the RGB image based approaches, we observe that \videolayout{} outperforms \monolayout{}, MonoOccupancy \cite{monooccupancy}  by considerable margins for all the evaluation metrics. The same can be also be observed in the results on KITTI RAW (\cf{}~Table~\ref{table:kittiraw}). 

% In all the splits, we observe \videolayout{} performs better than \cite{monolayout} as an effect of the enforced temporal constraints through the temporal consistency loss. \SaiShankar{temporal consistency's impact on map.} 
% Also, the increased scores for MonoLayout-ext over MonoLayout for weak supervision evidently show the effect of a better data preparation process \ref{seubsec:dataprep} over the simple sensor fusion approach used in \cite{monolayout}

\subsection{Vehicle Layout Estimation}

From Table~\ref{table:quantitative:main}, we can see that PseudoLidar-based methods have inferior performance in comparision to monocular methods\cite{monolayout, monooccupancy} on vehicle layout estimation. This can again be attributed to the fact that monocular depths are inprecise and sparse at large distances, which makes the PseudoLidar input unreliable for this task. 

Similar to road layout estimation, \videolayout{} performs better than \monolayout{} due to the temporal consistency loss and the adversarial regularization via the refinement network (\cf{} Fig.~\ref{fig:dynamic}). Also, MonoOccupany~\cite{monooccupancy} performs poorly on vehicle layout estimation, presumably due to \emph{blurriness} in the variational autoencoder used therein leading to low mAP scores.
% the inability of the variational autoencoder architecture(VAE) to predict sharp vehicle occupancies. 
% \SaiShankar{have to change the monoccupancy argument here}
% as the variational autoencoder-style architecture usually merges most of the vehicles into large bloblike structures

\subsection{Lane Layout Estimation}

We split the lane layout estimation into two tasks: \emph{ego-lane estimation} and \emph{overall lane detection}. This exclusive treatment of ego-lane estimation is due to its prominence in semi and fully autonomous driving.
% This is done to provide more emphasis on ego-lane estimation, which is essential for several autonomous driving tasks like trajectory prediction, object tracking, behavior planning etc.
Unlike objects, which can be ``detected" as bounding boxes, lanes are objects whose extents span potentially the entire width/height of the \bev{} image, and this calls for an appropriate evaluation protocol. We thus treat lane estimation akin to a ``segmentation" problem, and compare performance in terms of average precision and recall at varying IoU thresholds ($0.5$, $0.7$).
% For \emph{ego-lane estimation}, we see a similar trend. PseudoLidar-based approaches are outperformed by \monolayout{} and \videolayout{}.
% for the same reasons mentioned in Sec.~\ref{subsec:roadlayoutest}.
From Table~\ref{table:quantitative:main}, we see that that MonoOccupancy~\cite{monooccupancy} performs significantly better than PseudoLidar methods on ego-lane estimation.
% \SaiShankar{Reference to strong supervision}

\videolayout{} significantly outperforms other methods, owing to its ability to encode temporal information and the use of a separate refinement network. The refinement network corrects blobby lane estimates that do not match the true data distribution, resulting in performance boosts at higher IoU thresholds. A few qualitative results are presented in Fig.~\ref{fig:qualitative_road}.
% on ego-lane estimation task (\cf{}~Fig.~\ref{fig:qualitative_road}). We attribute this to the 
% From Table~\ref{table:quantitative:main} we can see that the performance of PseudoLidar-based methods drop significantly on the task of OverAll Lane detection task, this is because the lanes generated by the PseudoLidar based methods seldom cross the IoU threshold of 0.7. Also, the performance of \videolayout{}  increases dramatically on the IoU thresholded average precision metric. This can be purely attributed to the use of refinement network which removes the blobby lane detections that do not match the true data distribution leading to a significant increase in the $AP_{IoU>0.7}$.

% Table~\ref{table:ablation} analyzes the importance of sampling layer for static layout estimation. It can be seen that by adding the sampling layer to the static decoder performance increases for both \monolayout{}\cite{monolayout} and \videolayout{} architecture across all static layout estimation tasks. 
% \subsection{Amodal Scene Layout Estimation}
% Overall, we observe that \videolayout{} outperforms all the proposed methods and existing state of the art layout estimation techniques for road, vehicle, ego-lane as well as other lane layout estimation 
% % \Madhav{Where are the Tables etc for this section}

\begin{table}[]
    \centering
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{|c|c|c|c|c|}
        \hline  
                                      & \multicolumn{2}{c|}{Ego-Lane}     &  \multicolumn{2}{c|}{OverAll}       \\
        \cline{2-5}
        Method                        & mIOU        &  mAP               &  \small{$AP_{\small{iou>0.7}}$}    & \small{$R_{\small{iou>0.7}}$}   \\
        \hline
        VideoLayout (no samp., no reg.)   & $59.81$       &  $73.13$         &   $20.95$     &    $36.55$  \\
        VideoLayout (no reg.)             & $61.15$       &  $75.72$         &   $35.89$     &    $41.92$    \\
        VideoLayout (full)                & $62.68$       &  $76.80$         &   $38.56$     &    $44.33$           \\ 
        \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Analyzing effect of various subparts of the \videolayout{} architecture on Lane Layout estimation performance. The sampling layer and adversarial regularization improve performance.}
    \label{table:sampling} 
\end{table}


\begin{table}[]
    \centering
    \begin{adjustbox}{max width=\textwidth, totalheight=1.5cm}
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        Method              &  {\tiny \small{$AP_{\small{iou>0.5}}$}}  &   \small{$R_{\small{iou>0.5}}$} &  \small{$AP_{\small{iou>0.7}}$}   & \small{$R_{\small{iou>0.7}}$}   \\
        \hline
        PseudoLidar-UNet             & $19.32$       &  $43.24$         &   $8.53$     &     $19.09$  \\
        PseudoLidar-ENet             & $25.10$       &  $47.39$         &   $13.01$     &    $24.50$    \\
        MonoLayout\cite{monolayout}  & $25.38$       &  $55.06$         &   $16.09$     &    $34.91$           \\
        VideoLayout                  & $57.02$       &  $65.49$         &   $38.56$     &    $44.33$   \\
        \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Analyzing Lane layout scores at IoU thresholds of $0.5$ and $0.7$. $AP$ denotes average precision. $R$ denotes Recall. \videolayout{} consistently performs better across IoU thresholds.}
    \label{table:iou_thresh}
\end{table}



\subsection{Ablation Studies}

We conduct ablation studies to analyze the performance of various components in the pipeline. These lead to a number of interesting observations that we enlist below.

\subsubsection{Sensitivity of lane estimates to IoU thresholds}

In Table~\ref{table:iou_thresh}, we analyze the sensitivity of lane estimates to IoU thresholds. At lower thresholds ($AP_{IoU>0.5}$ and $R_{IoU>0.5}$), PseudoLidar-based techniques have similar performance to that of MonoLayout~\cite{monolayout}.
But as the threshold increases ($AP_{IoU>0.7}$ and $R_{IoU>0.7}$), PseudoLidar methods exhibit a dramatic performance drop, particularly in terms of recall.
We attribute this to the fact that PseudoLidar relies on monocular depth estimates which are sparse and inaccurate for vehicles farther from the camera.
On the other hand, \videolayout{} performs consistently across both IoU thresholds. Particularly at $AP_{IoU>0.5}$, we observe a significant performance increase compared to \monolayout{}.

% While in earlier results, we focus on $AP_{IoU>0.7}$ and $Recall_{IoU>0.7}$ as the metric for evaluating Overall lane detection. In Table \ref{table:iou_thresh}, we also look at $AP_{IoU>0.5}$ and $Recall_{IoU>0.5}$ to analyze the performance of the benchmark methods in more detail. It can be seen that for IoU threshold of 0.5 PseudoLidar based methods have similar performance to that of Monolayout\cite{monolayout} but their performance drops dramatically as IoU threshold is increased to 0.7 especially in terms of $Recall_{IoU>0.7}$. The reason behind this can be the fact that PseudoLidar based methods rely on monocular depth which gets sparser and more inaccurate as the distance from the ego-vehicle increases. Other observation that can be made from Table \ref{table:iou_thresh} is that \videolayout{} consistently performs well for both IoU thresholds, particularly $AP_{IoU>0.5}$ sees a significant bump in comparision to \monolayout{}\cite{monolayout}.  

\subsubsection{Effect of Sampling and Adversarial Refinement}

Table~\ref{table:sampling} shows the performance of different variants of \videolayout{} for lane layout estimation. \videolayout{} (no samp., no reg.) refers to a variant without a sampling layer in the static decoder and without adversarial regularization. \videolayout{} (no reg.) uses sampling layer in the static decoder. \videolayout{} (full) uses both sampling layer and an adversarial regularizer. It can be seen that each component meaningfully contributes to performance boosts.
% from Table \ref{table:iou_thresh} that performance of \videolayout{} improves by addition of each component.
The sampling layer enhances the capability of the model to capture the distribution of \emph{plausible} layouts, improving precision ($AP_{IoU>0.7}$).
The adversarial regularizer improves the sharpness of the predicted samples, improving the recall $R_{IoU>0.7}$.
% adding sampling layer $AP_{IoU>0.7}$ increases significantly which can be attributed to the model being more capable of modeling true distribution of conceivable lane layouts leading to less false positive lane predictions. As expected, adding the adversarial regularizer on top of the sampling layer enables the model to act more like a GAN and thus further improves the performance both in terms of $AP_{IoU>0.7}$ and $Recall_{IoU>0.7}$.



% \section{Discussion}

% \begin{figure}[!t]
%     \centering
%     \begin{adjustbox}{max width=\linewidth}
%     \begin{tabular}{ccc}
%         \toprule
%         % \midrule
%         \frame{\includegraphics[width=30mm,height=20mm]{images/rgb/0000000093.png}}
%         & \frame{\includegraphics[width=20mm,height=20mm]{images/pred/0000000093.png}}
%         & \frame{\includegraphics[width=20mm,height=20mm]{images/gt/0000000093.png}} \\
        
%         \frame{\includegraphics[width=30mm,height=20mm]{images/rgb/0000000021.png}} 
%          & \frame{\includegraphics[width=20mm,height=20mm]{images/pred/0000000021.png}}
%          & \frame{\includegraphics[width=20mm,height=20mm]{images/gt/0000000021.png}} \\
         
%           \frame{\includegraphics[width=30mm,height=20mm]{images/rgb/0000000134.png}}
%          & \frame{\includegraphics[width=20mm,height=20mm]{images/pred/0000000134.png}}
%          & \frame{\includegraphics[width=20mm,height=20mm]{images/gt/0000000134.png}} \\
%         \midrule
%         RGB & \videolayout{} & \textit{GroundTruth} \\

%         \bottomrule
%         % \textbf{RGB} & \textbf{w/o Discrim.} & \textbf{With Discrim.} & \textbf{GT}
%     \end{tabular}
%     \end{adjustbox}
%     \caption{\footnotesize{\textbf{Failure Cases} of \videolayout{}. (\emph{Top row}) Failure to predict ego-lane. (\emph{Middle row}) Failure in heavy traffic scenarios. (\emph{Bottom row}) Failure in predicting lane width. 
%     % row 3 shows the case where \videolayout{} fails to predict the lane-width accurately.
%     }}
%     % \Kaustubh{add caption}
    
%     % \caption{Qualitative comparison on KITTI\cite{KITTI} for showing the effect of discriminator on road layouts. For each row, the first image is a RGB image in KITTI dataset. The second image in the row is representative of the output generated by \monolayout{} without discriminator. The third image in the row is the output generated by \monolayout{} in the presence of a discriminator. The final image in the row is the corresponding manually annotated ground truth road layout}
%     \label{fig:failure}
% \end{figure}

\begin{figure}[!t]
    \centering
    \begin{adjustbox}{max width=\linewidth}
    \includegraphics[]{images/failure_cases.png}
    \end{adjustbox}
    \caption{\footnotesize{\textbf{Failure Cases} of \videolayout{}. (\emph{Top row}) Failure to predict ego-lane. (\emph{Middle row}) Failure in heavy traffic scenarios. (\emph{Bottom row}) Failure in predicting lane width. }}
    \label{fig:failure}
\end{figure}


\subsection{Failure cases}

Despite its impressive performance, \videolayout{} fails in multiple scenarios. A few representative failure cases are shown in Fig.~\ref{fig:failure}. Often, such failures are due to high-dynamic range conditions, where shadows are mistaken for lanes, or in heavy traffic scenarios.

\subsection{Runtime}

On an NVIDIA RTX 1080Ti, the inference rate of \videolayout{} is slightly over $40$ frames per second, which is suitable for real-time performance.
% significantly faster than pseudolidar-based methods ($< 1.8$ fps), and comparable to MonoOccupancy~\cite{monooccupancy} ($15$ fps), but is far inferior to \monolayout{} ($32$ fps).

\section{Conclusion}

Amodal layout estimation is an emerging perception task for autonomous driving. Solving this task necessitates an understanding of not just entities present in an image, but also a reasoning of occluded portions. Benchmarks have driven progress in allied perception tasks such as object detection, segmentation, tracking, depth estimation, and more. In that spirit, we introduce a new benchmark (\coolname{}) for amodal layout estimation. We implement several baselines and prior art, and make all our code and data available. We further propose \videolayout{}, a simple yet effective technique, and demonstrate that reasoning about image sequences leads to coherent and robust layout estimates. We hope the dataset and benchmark serve as a breeding ground for a new class of approaches that will take us a step closer to understanding the 3D world from a sequence of its projections.

% Th paper advances the state of the art in the following ways. First, it releases a dataset catered to amodal scene layout estimation that is distinct from current datasets that provide for semantic segmentation, object detection detection, tracking and trajectory prediction. The dataset, \emph{AutoLay} provides annotation of road, lane instances in the road, vehicles, sidewalk and crosswalks for 3D Lidar points as well as layout occupancy map in \bev{}. Second it benchmarks Amodal Layout Estimation across a variety of methods that include recent works such as \cite{monolayout, monooccupancy} and across a variety of tasks including road layout estimation, vehicle layout estimation, ego-lane layout estimation and overall lane detection. Third it establishes the superiority of the method proposed in the paper, \videolayout{} as a consequence of its ability to integrate temporal data and the consistency loss function proposed in the paper.

